Randomness Efficient Fast-Johnson-Lindenstrauss Transform with Applications in Differential Privacy and Compressed Sensing

The Johnson-Lindenstrauss property ({\sf JLP}) of random matrices has immense application in computer science ranging from compressed sensing, learning theory, numerical linear algebra, to privacy. This paper explores the properties and applications of a distribution of random matrices. Our distribution satisfies {\sf JLP} with desirable properties like fast matrix-vector multiplication, sparsity, and optimal subspace embedding. We can sample a random matrix from this distribution using exactly $2n+n \log n$ random bits. We show that a random matrix picked from this distribution preserves differential privacy under the condition that the input private matrix satisfies certain spectral property. This improves the run-time of various differentially private mechanisms like Blocki {\it et al.} (FOCS 2012) and Upadhyay (ASIACRYPT 13). Our final construction has a bounded column sparsity. Therefore, this answers an open problem stated in Blocki {\it et al.} (FOCS 2012). Using the results of Baranuik {\it et al.} (Constructive Approximation: 28(3)), our result implies a randomness efficient matrices that satisfies the Restricted-Isometry Property of optimal order for small sparsity with exactly linear random bits. We also show that other known distributions of sparse random matrices with the {\sf JLP} does not preserves differential privacy; thereby, answering one of the open problem posed by Blocki {\it et al.} (FOCS 2012). Extending on the works of Kane and Nelson (JACM: 61(1)), we also give unified analysis of some of the known Johnson-Lindenstrauss transform. We also present a self-contained simplified proof of an inequality on quadratic form of Gaussian variables that we use in all our proofs.

==> appendices.tex <==
\begin{versionA}
\section{Some Known Inequalities and Results}
In this appendix, we present some of the known inequalities and results we used in the paper.
\subsection{Some Known Inequalities}
We use few well known concentration bounds for random subgaussian variables at various points of our proof. The following is the multiplicative form of the Hoeffding's inequality. 
\begin{theorem} {\em (Hoeffding's inequality)} \label{thm:ch}
Let $X_1, \cdots, X_n$ be $n$ independent  random variables with the same probability distribution, each ranging over the real interval $[i_1, i_2]$, and let $\mu$ denote the expected value of each of these variables. Then, for every $\varepsilon >0$, we have
\[ \p \sparen{ \left| \frac{\sum_{i=1}^n X_i}{n} - \mu \right| \geq \varepsilon } \leq 2 \exp \paren{- \frac{2\varepsilon^2n}{(i_2-i_1)^2} }.  \]
\end{theorem} 
The Chernoff-Hoeffding bound is useful for estimating the average value of a function defined over a large set of values, and this is exactly where we use it. Hoeffding showed that this theorem holds for sampling without replacement as well. However, when the sampling is done without replacement, there is an even sharper bound by Serfling~\cite{Serfling74}.

\begin{theorem} {\em (Serfling's bound)} \label{thm:serfling}
Let $X_1, \cdots, X_n$ be $n$ samples drawn without replacement from a list of $N$ values, each ranging over the real interval $[i_1, i_2]$, and let $\mu$ denote the expected value of each of these variables. Then, for every $\varepsilon >0$, we have
\[ \p \sparen{ \left| \frac{\sum_{i=1}^n X_i}{n} - \mu \right| \geq \varepsilon } \leq 2 \exp \paren{- \frac{2\varepsilon^2n}{(1-(n-1)/N)(i_2-i_1)^2} }.  \]
\end{theorem} 
The quantity $1-(n-1)/N$ is often represented by $f^*$. Note that when $f^*=0$, we derive~\thmref{ch}. Since $f^* \leq 1$, it is easy to see that~\thmref{serfling} achieves better bound than~\thmref{ch}.

We also use the following result of Hanson-Wright~\cite{HW} for subgaussian random variables.
\begin{theorem} {\em (Hanson-Wright's inequality).} \label{thm:hw}
	For any symmetric matrix $\bA$, sub-gaussian random vector $\bx$ with mean $0$ and variance $1$, 
	\begin{align} \p_{\mathbf{g}} \sparen{ | \mathbf{g}^{\mathsf T} \bA \mathbf{g} - \tr(\bA) | > \eta } \leq 2 \exp \paren{ -\min \set{ {c_1 \eta^2}/{\|\bA\|_F^2} , {c_2 \eta}/{\|\bA\|}} }. \label{eq:hw} \end{align}
\end{theorem}
The original proof of Hanson-Wright inequality is very simple when we only consider special class of subgaussian random variables. We give the proof when $\mathbf{g}$ is a random Gaussian vector in~\appref{gaussian}. A proof for $\sber(1/2)$ is also quite elementary. For a simplified proof for any subgaussian random variables, we refer the readers to~\cite{RV}.


\subsection{Some Known Results}
The following result was shown by Ailon and Chazelle~\cite{AC09}.
\begin{theorem} \label{thm:AC09}
Let $\bW$ be a $n \times n$  Hadamard matrix and $\bD$ be a diagonal signed Bernoulli matrix with $\bD_{ii} \sim \sber(1/2).$ Then for any vector $\bx \in \bS^{n-1}$, we have 
\[ \p_D \sparen{\| \bW \bD\bx\|_\infty \geq \sqrt{\paren{\log (n/\delta)}/{n}}} \leq \delta. \]
\end{theorem}

The equivalence of {\sf JLP} and {\sf RIP} was proven by two separate works. Baranuik {\it et al.}~\cite{BDDW07} first showed that {\sf RIP} implies {\sf JLP}.
\begin{theorem} \label{thm:BDDW07}
	Let $\bPhi$ be a $r \times n$ random matrix  drawn according to any distribution that satisfies~\eqnref{JL}. Then, for any set $T$ with $|T|=k<n$ and any $0\leq \delta \leq 1$, we have $ \forall x \in X_T$
	\[ \p_\bPhi [ (1-\delta) \| \bx \|_2 \leq \| \bPhi_T \bx \|_2 \leq (1+\delta) \| \bx \}_2] \geq 1 - 2(12/\varepsilon)^k e^{-O(\delta n)},\]  where $X_T$ is all $\bx \in X$ restricted to indices in the set $T$.
	Moreover,  the $\mathsf{RIP}$ holds for $\bPhi$ with the prescribed $\delta$ for any $s \leq O\paren{ {\delta^2r}/{\log (n/r)}} $ with probability at least $1- 2e^{-O(r)}$.
\end{theorem} 

The converse was shown in a beautiful paper by Krahmer and Ward~\cite{KW11}.

\begin{theorem} {\em (\cite[Proposition 3.2]{KW11})} \label{thm:KW11}
	Let $\varepsilon$ be an arbitrary constant. Let $\bPhi$ be a matrix of order $k$ and dimension $r \times n$ that satisfies the relation $k \leq c_1 \delta_k^2 r / \log (n/r)$ and has {\sf RIP}. Then the matrix $\bPhi \bD$, where $\bD$ is an $n \times n$ diagonal matrix  formed by Rademacher sequence, satisfies~\eqnref{JL}.
\end{theorem} 

In one of our proofs of differential privacy, we prove that each row of the published matrix preserves $(\alpha_0, \beta_0)$-differential privacy for some appropriate $\alpha_0,\beta_0$, and then invoke a composition theorem proved by Dwork, Rothblum, and Vadhan~\cite{DRV10} to prove that the published matrix preserves $(\alpha,\beta)$-differential privacy. The following theorem is the composition theorem that we use.
\begin{theorem} \label{thm:DRV10}
	Let $\alpha_0, \beta_0 \in (0,1)$, and $\beta'>0$. If $\mathfrak{M}_1, \cdots , \mathfrak{M}_\ell$ are each $(\alpha_0, \beta_0)$-differential private mechanism, then the mechanism $\mathfrak{M}(D):= (\mathfrak{M}_1(D), \cdots , \mathfrak{M}_\ell(D))$ releasing the concatenation of each algorithm is $(\alpha, \ell \beta_0+\beta)$-differentially private for $\alpha < \sqrt{2\ell \ln (1/\beta)}\alpha_0 + 2\ell \alpha^2_0$.
\end{theorem}

\section{Missing Proofs} \label{app:missing}
\subsection{Proof of~\lemref{P_2}} \label{app:P_2}
Let  $t=n/r$. 
Fix $1\leq j \leq r$. Let $\by =\bW \bD \bx$.
Let $\by'=  \bPi \by$ and $\bz_{(j)} = \sqrt{n/t} \paren{\by'_{(j-1)n/r+1}, \cdots , \by'_{jn/r+1}}$. Therefore, $\|\bz_{(j)}\|^2_2 = (n/t)\sum_{i=1}^t \by_{(j-1)t+i}'^2$. From~\thmref{AC09}, we know that $\|\bz_{(j)}\|_\infty$ is bounded random variable with entries at most $\sqrt{\log(n/\delta)/t}$ with probability $1-\delta.$
Also, $\E_{\bP_2,\bPi}[\|\bz_{(j)}\|^2]=1$. Since this is sampling without replacement; therefore, we use the  Serfling bound~\cite{Serfling74}. Applying the bound gives us
\begin{align}
 \p_{\bPi} \sparen{ \left|~\left\| \bP_2 \bPi \by \right\|_2^2 - 1 \right| \geq \varepsilon  } = \p \sparen{ | \|\bz_{(j)}\|_2^2 - 1 | > \varepsilon } \leq 2\exp(-\varepsilon^2 t / \log(n/\delta)). \label{eq:P_2_1} \end{align}


%Fix $1\leq j \leq r$. Let $\by = \sqrt{n/t} \bW \bD \bx$. Let $\by'=  \bPi \by$ and $\bz^{(j)} =\paren{\by'_{(j-1)t+1}, \cdots , \by'_{jt+1}}$. Therefore, $\|\bz^{(j)}\|^2_2 = \sum_{i=1}^t (\bz_i^{(j)})^2$. From~\thmref{AC09}, we know that $\|\bz^{(j)}\|_\infty$ is bounded random variable with entries at most $\sqrt{\log(n/\delta)/t}$ with probability $1-\delta.$ Also, $\E_{\bP_2,\bPi}[\|\bz^{(j)}\|^2]=1$. Since this is sampling without replacement; therefore, we use the  Serfling bound~\cite{Serfling74}. Applying the bound gives us
%\begin{align}\p \sparen{ | \|\bz^{(j)}\|_2^2 - 1 | > \varepsilon } \leq 2\exp(-\varepsilon^2 t / \log(n/\delta)). \label{eq:P_2_1} \end{align}

In order for~\eqnref{P_2_1} to be less than $\delta/r$, we need to evaluate the value of $t$ in the following equation:
\[ \frac{\varepsilon^{-2} t}{\log (n/\delta)} \geq \log \paren{\frac{2r}{\delta}} \quad \Rightarrow \quad t \geq \varepsilon^2 \log (n/\delta) \log(2r/\delta).  \]

%In order to solve the above expression, it is first reasonable to consider the equation of the form $\exp(x) \geq \lambda x.$ If $\lambda \leq e$, then the above expression is true for all values of $x$. If $\lambda > e$, we have two ranges of $x$ for which  $\exp(x) \geq \lambda x$ and we need to solve the two values. For this, we solve the following equation: $f(x):=\exp(x) - \lambda x$. It is easy to see that for $x=\log \lambda$, $f(x) <0$. On the other hand when $x=2\log \lambda$, we have that $f(x)>0$. In other words, there is some value in the range $[\log \lambda, 2 \log \lambda]$ which is the solution of $f(x)=0$ and any $x$ greater than the root of this expression is a valid solution for $x$. 

%Returning to our problem, we have $\exp(t) \geq \exp(\varepsilon^2) \paren{\frac{t}{\delta}}^{\log (n/\delta)}$. Proceeding as above, we have to worry only when 
%\begin{align} \exp(\varepsilon^2) \delta^{-\log(n/\delta)} \geq \exp(1) \quad \Rightarrow \quad \varepsilon^{2} \geq c_1 \delta \log (n/\delta). \label{eq:P_2} 
%\end{align} for a universal constant $c_1.$ For the latter, we can follow the same logic as above to say that it holds for all $t \geq c_2 \varepsilon^{-2} \log (n/\delta) \log (1/\delta)$ for a large constant $c_2.$ 
The inequality is trivially true for $t=n/r$ as long as $t \leq n^{1/2+\tau}$ for some arbitrary constant $\tau >0$ as shown in~\figref{basic}.
Now for this value of $t$, we have for a fixed $j \in [t]$
\begin{align}\p \sparen{ | \|\bz_{(j)}\|_2^2 - 1 | > \varepsilon } \leq \exp(-\varepsilon^2 t / \log(n/\delta)) \leq \delta/r. \end{align}

%Using union bound, we have the result. For this to be less than $\delta$, pick $t = \varepsilon^{-2} \log(1/\delta) \log(n/\delta).$

Using union bound over all such possible set of indices gives the lemma.%, we get that  $\p \sparen{ \left| \| P_2 \bPi WD \bx \|-1 \right| \geq \varepsilon } \leq \delta.$

\subsection{Proof of~\lemref{gaussian}} \label{app:P_1}
Let $\mathbf{g} $ be the vector corresponding to the matrix $\bP_1$, i.e., $\mathbf{g}_k = (\bP_1)_{ij}$ for $k=(i-1)t +j$. Let $\bz_{(1)}, \cdots, \bz_{(r)} \in \bS^{t-1}$ be $r$ vectors of dimension $t$. Let $\bA$ be the matrix formed by diagonal block matrix each of which has the form $\bz_{(i)} \bz_{(i)}^{\mathsf T}/r$ for $1\leq i \leq r$. Therefore, $\tr(\bA)=1$, $\|\bA\|_F^2 = 1/r$. Also, since the only eigen-vectors of the constructed $\bA$ is $\begin{pmatrix} \bz_{(1)} & \cdots & \bz_{(r)} \end{pmatrix}^{\mathsf T}$, $\|\bA\|=1$. Plugging these values in the result of~\thmref{hw}, we have 
\begin{align} \p_{\mathbf{g}} \sparen{ | \mathbf{g}^{\mathsf T} \bA \mathbf{g} - 1 | > \varepsilon } \leq 2 \exp \paren{ -\min \set{ \frac{c_1 \varepsilon^2}{1/r} , {c_2 \varepsilon}} } \leq \delta. \label{eq:gaussian} \end{align}
for $r=O(\varepsilon^{-2} \log (1/\delta))$. It is easy to check that $\mathbf{g}^{\mathsf{T}}\bA \mathbf{g} = {\frac{1}{r}}\| \bP_1 \bx \|_2^2$. This completes the proof.

\subsection{Proof of~\thmref{newgaussian}} \label{app:newgaussian}
\thmref{AC09} gives us that for any $\bx \in \bS^{n-1}$, $\sqrt{n/t} \| \bW \bD \bx \|_\infty \leq \sqrt{\log (n/\delta)/t}$ with probability $1-\delta$. Further,~\lemref{P_2} gives us that if $\bP_2 \bPi$ is fed with an input $\by = \sqrt{n/t} \bW \bD \bx$, then we have a set of $t$-dimensional vectors $\bz_{(1)}, \cdots, \bz_{(r)}$ such that each of them have Euclidean norm between $1-\varepsilon$ and $1+\varepsilon$. Using $\bz_{(1)}, \cdots, \bz_{(r)}$ to form the matrix $\bA$ as in the proof of~\lemref{gaussian},  we have $\| \bA \|_F^2 \leq (1+\varepsilon)^2/r$ and $\|A\| \leq (1+\varepsilon).$ Therefore, using~\thmref{hw}, we have
\begin{align} \p_{\mathbf{g}} \sparen{ | \mathbf{g}^{\mathsf T} \bA \mathbf{g} - 1 | > \varepsilon } \leq 2 \exp \paren{ -\min \set{ \frac{c_1 r \varepsilon^2}{(1+\varepsilon)^2} , \frac{c_2 \varepsilon}{(1+\varepsilon)}} } \leq \delta . \end{align}

For this to be less than $\delta$, we need $r \leq \frac{c'(1+\varepsilon)^2}{\varepsilon^2} \log \paren{\frac{1}{\delta}} \leq 4c' \varepsilon^{-2} \log(1/\delta)$. As before, it is easy to check that $\mathbf{g}^{\mathsf{T}}\bA \mathbf{g} = {\frac{1}{r}}\| \bP_1 \bx \|_2^2$.

\subsection{Proof of~\lemref{zero}} \label{app:zero}
Let us denote by $t=n/r$. From~\thmref{AC09}, we know that $\bW \bD \bx$ is bounded random variable with entries at most $\sqrt{(\log(n)+n^{1/3})/n}$ with probability $1-2^{-c_3n/3}.$   Let $\by= \bPi \bW \bD \bx$, and  $\by^{(j)} = \sqrt{n/t}(\by_{(j-1)t+1}, \cdots, \by_{jt})$

Fix a $j$. First note that $\E[\|\by^{(j)}\|^2]=1$. Since the action of $\bPi$ results in sampling without replacement; therefore, Serfling's bound~\cite{Serfling74} gives
\begin{align*}
\p \sparen{ \left\| \by^{(j)} \right\|_2^2  \leq 1- \zeta } \leq \exp \paren{-\frac{\zeta^2 n }{ \log(n)+n^{1/3}}} \leq \exp(- c_3' \zeta^2 n^{2/3}).
 \end{align*}
 for $\zeta <1$.
Setting $\theta = 1-\zeta$ and using union bound over all $r$ gives the lemma. 


\end{versionA}


==> application.tex <==
\subsection{Johnson-Lindenstrauss and Compressed sensing}
 In the domain of compressed sensing, Candes and Tao~\cite{CT06} and Candes, Rohenberg, and Tao~\cite{CRT06} introduced a closely related property of a projection matrix called  {\em Restricted Isometry Property} ($\mathsf{RIP}$). More concretely, they defined $\mathsf{RIP}$ as follows.
\begin{definition} \label{defn:RIP}
	Given any set $T \subseteq \{1, \cdots, r\}$, we say that an $r \times n$ matrix $\Phi$ satisfies the {\em Restricted Isometry Property}  of {\em order} $k$ if there exists a $0<\delta_k<1$ such that 
	\begin{equation} 
	  (1-\delta_k) \| \bx_T\|_2^2 \leq \|\Phi_T \bx_T \|_2^2 \leq (1+\delta_k) \| \bx_T\|_2^2 \label{eq:RIP}
	 \end{equation}
	  holds for all set $T$ with $|T|<k$ with high probability, where $\Phi_T$ ($\bx_T$, respectively) is the restriction of $\Phi$ ($\bx$, respectively) to the indices in $T$. The {\em restricted isometry  constant} of { order} $k$ is the smallest $\delta$ for which~\eqnref{RIP} holds.
\end{definition}

%It was shown by Candes and Tao~\cite{CT06} that if $\delta_k + \delta_{2k} + \delta_{3k} < 1$, then one can recover any sparse signal $\bx_s$ with support size obeying $|T|<k$ by solving the following linear program:$  \min \| \bx\|_1, \text{ subject to }   \Phi \bx =y .$

The similarity in~\eqnref{JL} and~\eqnref{RIP} is quiet evident and suggests some connection between both these properties of random matrices. Baraniuk {\it et al.}~\cite{BDDW07} were the first to show a relation between these two properties of random projection matrices.  More concretely, they showed the following.
\begin{theorem} {\em (Baraniuk {\it et al.}~\cite{BDDW07}).} \label{thm:BDDW07}
	Let $\Phi$ be a $r \times n$ random matrix  drawn according to any distribution that satisfies~\eqnref{JL}. Then, for any set $T$ with $|T|=k<n$ and any $0\leq \delta \leq 1$, we have $ \forall x \in X_T$
	\[ \p [ (1-\delta) \| \bx \|_2 \leq \| \Phi_T \bx \|_2 \leq (1+\delta) \| \bx \}_2] \geq 1 - 2(12/\varepsilon)^k e^{-O(\delta n)},\]  where $X_T$ is all $\bx \in X$ restricted to indices in the set $T$.
	Moreover,  the $\mathsf{RIP}$ holds for $\Phi$ with the prescribed $\delta$ for any $k \leq O\paren{ {\delta^2r}/{\log (n/r)}} $ with probability at least $1- 2e^{-O(r)}$.
\end{theorem} 

Ailon and Liberty~\cite{AL13} proved the converse for a special case and by Krahmer and Ward~\cite{KW11} proved for the general case. More concretely, the authors proved the following.
\begin{theorem} {\em (Krahmer-Ward~\cite[Proposition 3.2]{KW11})} \label{thm:KW11}
	Let $\varepsilon$ be an arbitrary constant. Let $\Phi$ be a matrix of order $k$ and dimension $r \times n$ that satisfies the relation $k \leq c_1 \delta_k^2 r / \log (n/r)$ and~\eqnref{RIP}. Then the matrix $\Phi D$, where $D$ is an $n \times n$ diagonal matrix  formed by Rademacher sequence, satisfies~\eqnref{JL}.
\end{theorem} 

Baranuik {\it et al.}~\cite{BDDW07} showed that the choice of $k$ used in above theorem is optimal through the Gelfand's width argument.  However, to our knowledge, there is no  construction of random matrices that satisfies $\mathsf{RIP}$  of optimal order and allows fast matrix-vector multiplication. 

For the rest of this exposition, we restrict our attention to random projection matrices that allows fast matrix-vector multiplication and uses linear sampling. We can  widely divide the class of such projection matrices into following two groups depending on how the matrices are chosen: either the original matrix is chosen from some known class of matrix and each row is chosen uniformly at random (bounded-orthogonal system), or the first row of matrix is chosen at random and the remaining rows are formed in some deterministic manner (partial circulant matrices). In the former case, the best known bound is $r \geq \delta^{-2} k \log^4n$ due to~\cite{CT06, RV08}, and in the case of latter case, the best known bound is $r \geq \max ({ \delta^{-1} \sqrt{(k \log n)^3}, \delta^{-2} k \log^4 n })$~\cite{RRT10}. Recently, Neilson, Price, and Wooters~\cite{NPW14} improved these  bounds to $r=O(\delta^{-1}k \log n \log^2(k \log n))$ at the cost of increased random samples. 
It is clear that all these works achieves Restricted Isometry of sub-optimal order. 

The above discussion raises the following natural  question:
{\em	Is there a distribution of random matrices that achieves the $\mathsf{RIP}$ of optimal order using linear random samples?} We answer it partially by achieving a bound on $r$ which is $O(\log^3 n)$ factor better than~\cite{RRT10} and $O(\log^2(k \log n))$ factor better than~\cite{NPW14} (refer to Table~\ref{tableRIP}), and a bound on $k$ which is suboptimal by $\log n$ factor. We use a complementary approach, i.e., we give an unconditional construction of projection matrices that satisfies the {\sf JL} bound and then invoke~\thmref{BDDW07} whereas previous works used a distribution of  matrices that satisfies $\mathsf{RIP}$ to give a distribution of matrices that satisfies the {\sf JL} bound. 

\begin{table} [t]
{\small
{
\begin{tabular}{|c|c|c|c|}
\hline
Ensembles & 	Number of rows &	Multiplication time & Random samples \\ \hline
Bounded-orthogonal~\cite{CT06,RV08} & $O(\delta^{-2} k \log^4n)$ & $O(n \log n)$ & \textcolor{blue}{$O(n) $}\\ \hline
Partial circulant~\cite{RRT10}	& $\max ({ \delta^{-1} \sqrt{(k \log n)^3}, \delta^{-2} k \log^4 n })$ & \textcolor{blue}{$O(n \log r)$} & \textcolor{blue}{$O(n) $} \\ \hline
Hash-partial matrices~\cite{NPW14} & $O(\delta^{-1} k \log n \log^2(k \log n))$ & \textcolor{blue}{$O(n \log r) + {O}(r \log^c n)$} & $O(rn) $ \\ \hline
This work &  \textcolor{blue}{$O(\delta^{-1} k \log n)$} & $O(n \log n)$ & \textcolor{blue}{O(n)} \\ \hline
\end{tabular} \label{table:compare}
\caption{Comparison between our $\mathsf{RIP}$ bound with previous bounds (text in blue is the best in respective category).}  \label{tableRIP}
}}\end{table}


\subsection{Johnson-Lindenstrauss and Differential Privacy} In the recent past, {\em differential privacy} has emerged as  very robust guarantee of privacy. Formally it is defined as follows. 
\begin{definition} \label{def:approxdp}
	A randomized mechanism, $\cK$, gives {\em $(\varepsilon, \delta)$-differential privacy}, if for all  
data-sets $D_1$ and $D_2$ with $\|D_1 -D_2\| \leq 1$, and all range $S \subset Range(\cK)$, 
		$ \p[\cK(D_1) \in S] \leq \exp (\varepsilon) \p[\cK(D_2) \in S] + \delta, $ where the probability is over the coin tosses of $\cK$. When $\delta=0$, we get the traditional definition of {\em differential privacy}.
\end{definition}

Blocki {\it et al.}~\cite{BBDS12} showed that {\sf JL} transform with random Gaussian matrices  preserves { differential privacy}. They left the question open {\em whether other constructions of {\sf JL} transform preserves differential privacy or not (more specifically, the fast-{\sf JL} transform and sparse-{\sf JL} transform)}. In this paper, we show that our construction of {\sf JL} transform also preserves differential privacy. Our construction is sparse (in terms of random sampling) and fast; thereby giving an affirmative answer to their question. The case why the number of random sample is important is exemplified by recent works of Chaudhary {\it et al.}~\cite{CSS12}, Mironov~\cite{Mironov12}, Kapralov and Talwar~\cite{KT13}. In Table~\ref{table}, we compare various aspects of our results with the known mechanisms. 

%One of the reasons why the proof of Blocki {\it et al.}~\cite{BBDS12} does not generalize to any {\sf JL}-transform is its strong dependency on the fact that each samples in a dense Gaussian matrices is picked i.d.d. More concretely, they  each row of their published matrix is a multivariate Gaussian and preserves differential privacy. They then invoke the composition theorem of Dwork, Rothblum and Vadhan~\cite{DRV10} to prove differential privacy of the entire published matrix. Unfortunately, we cannot invoke the composition theorem.
%The reason why Blocki {\it et al.}~\cite{BBDS12} could invoke the composition theorem and we cannot is due to the independence of every row of their projection matrix. On the other hand, our resulting projection matrix reuses random samples. Therefore, applying our projection matrix to a private matrix does not yield $n$ independent multivariate distribution, but rather one matrix-variate distribution. We compute the resulting distribution and then prove that it preserves differential privacy. For that, we have to bound the trace of a sample from a $\chi^2$-distribution. 

\begin{table} [t]
{\small
{
\begin{tabular}{|c|c|c|c|c|}
\hline
Method & Cut-queries & Covariance-Queries & Run-time & $\#$ Random Samples \\ \hline
Randomized Response~\cite{BDMN05,GRU12} & $O(\sqrt{sn \log \kappa/\varepsilon})$ & $\tilde{O}(\sqrt{d \log \kappa}/\varepsilon)$ & \textcolor{blue}{$\Theta(n^2)$} & $O(n^2)$ \\ \hline
Exponential~\cite{BLR08,MT07}& $O(n \log n /\varepsilon)$ & $O(n \log n /\varepsilon)$ & Intractable & $O(n^2)$\\ \hline
Multiplicative Weight~\cite{HR10} & $\tilde{O} (\sqrt{|\cE(\cG)|} \log \kappa /\varepsilon)$  & $\tilde{O}(d \sqrt{n \log \kappa/\varepsilon})$ & $O(n^2)$ & $O(n^2)$ \\ \hline
Johnson-Lindenstrauss~\cite{BBDS12} & \textcolor{blue}{$O(s \sqrt{\log \kappa}/\varepsilon)$} & \textcolor{blue}{$O(\varepsilon^{-2}\log \kappa)$} & $O(n^{2.38})$ & $O(rn)$ \\ \hline
Graph Sparsification~\cite{Upadhyay13} & \textcolor{blue}{$O(s \sqrt{\log \kappa}/\varepsilon)$} & $-$ & $O(n^{2+o(1)})$ & $O(n^2)$ \\ \hline
This paper &  \textcolor{blue}{$O(s  \sqrt{\log \kappa}/\varepsilon)$} & \textcolor{blue}{$O(\varepsilon^{-2}\log \kappa)$} & $O(n^2 \log n)$ &  \textcolor{blue}{$3n$} \\ \hline
\end{tabular} \label{table:compare}
\caption{Comparison between our mechanism and other mechanism (text in blue is the best in respective category).}  \label{table}
}}\end{table}

\subsection{Johnson-Lindenstrauss and Functional analysis} Due to the usefulness of the {\sf JL} transform, there has been considerable effort by researchers to prove such a dimensionality reduction theorem in other normed spaces. All of these efforts have thus far resulted in negative results which show that the {\sf JL} lemma fails to hold true in certain non-Hilbertian settings. More specifically, Charikar and Sahai~\cite{CS02} proved that there is no dimension reduction via linear mappings in $\ell_1$-norm. This was extended to the general case by Johnson and Naor~\cite{JN10}. They showed that a normed space that satisfies the {\sf JL} transform is very close to being Euclidean in the sense that all its subspaces are close to being isomorphic to Hilbert space. 
Recently, Allen-Zhu, Gelashvili, and Razenshteyn~\cite{AGR14} showed that there does not exists a projection matrix with $\mathsf{RIP}$ of optimal order for any $\ell_p$ norm other than $p=2$. In the view~\thmref{KW11} and characterization by Johnson and Naor, our result gives an alternate reasoning for their impossibility result. Moreover, using the result by Pisier~\cite{Pisier}, which states that, if a Banach space has Banach-Mazur distance  $o(\log n)$, then the Banach space is super-reflexive, we get one such space using just linear samples. This has many applications in Functional analysis (see~\cite{Conway} for details).

\subsection{Previous Works}
The amount of work to construct projection matrices that satisfies {\sf JL} lemma is so wide that we cannot hope to include all of them in full detail here. Hence, we include a partial list of  works that are most closely related to ours.  We refer to Matousek~\cite{Matousek08} for a better exposition of the variants of {\sf JL} transform.

%The first major attempt to improve the computational time of performing the {\sf JL} mapping was done by Ailon and Chazelle~\cite{AC09}. They used the idea of preconditioning the input so that the $\ell_2$ norm is maintained and individual coordinates of the preconditioned input is bounded. Their idea of preconditioning input was used in many later works as well, more specifically the works that gave sparser variants of {\sf JL} transform, like Dasgupta et al~\cite{DKS10} and Kane and Neilson~\cite{KN12, KN14}, and the works that gave dense-{\sf JL} transform~\cite{LAS08}. The main advantage of sparse-{\sf JL} transform is its fast computation. Unfortunately, their randomness complexity is always high.

%On the other hand, the question of less random sampling was considered by Ailon and Liberty~\cite{AL09}. They proposed a projection matrix that achieves the required distortion condition by using Rademacher variables and dual-BCH codes. Subsequently, Hinrichs and Vybiral~\cite{HV11} proved the similar result using partial circulant matrices. Since then, several results using partial circulant matrices that achieves better bound have been proposed~\cite{Vybiral, ZC13}. In parallel, there have been works to reduce the amount of random sampling required to construct the {\sf JL} transform, most notably by Krahmer and Ward~\cite{KW11} and Ailon and Liberty~\cite{AL13}.


The original {\sf JL} transform used spherical symmetry of the distribution, i.e., the random projection matrix $\Phi$ satisfies the following property: the distribution of $\Phi A$ and $\Phi$ are same for every orthogonal matrix $A$. Another key aspect of the original construction was that the rows of the projection matrix are orthonormal.  The original proof relied on both these properties. %An inherent drawback of the construction was that the distribution was over dense matrices.
Achlioptas~\cite{Achlioptas03} observed that we only need $(\Phi_{i:} \bx)^2$ to be concentrated around the mean for all unit vectors, where $\Phi_{i:}$ is the $i$-th row of matrix $\Phi$. It is not difficult to see that this property is satisfied by any matrix that has spherical symmetry. The motivation for Achlioptas~\cite{Achlioptas03} was to use a matrix that is easier to use in practice, so he picked each entry of the matrix from a Rademacher sequence. The final matrix was constructed by normalizing rows.  

In both the variants, the distribution is over dense random matrices. Therefore, for any vector $x$, performing an embedding takes time proportional to both the size of the matrix and its $\ell_0$-norm. This is specially unfortunate for the application in streaming algorithms and large-data analysis, two of the main applications of {\sf JL} transform. Therefore, in the last decade, from the view point  of these applications, the main research direction was concentrated on performing this mapping in an ``efficient" manner. 

One obvious way to improve the efficiency of the projection is to make the projection matrix sparse. Achlioptas~\cite{Achlioptas03} already achieves a one-third factor improvement in the sparsity parameter of the projection matrix. Subsequently, works like \cite{TZ04} gave distribution over matrices with only  $O(\log (1/\delta))$ non-zero entries in every column, but they do not provide an embedding in to $\ell_2$. The first major breakthrough in this came through the work of Dasgupta, Kumar, and Sarlos~\cite{DKS10}, who gave a distribution over projection matrix with only $\tilde{O}(\varepsilon^{-1} \log ^3(1/\delta))$ non-zero entries in every column. Subsequently, Kane and Nelson~\cite{KN12, KN14} improved it to $\Theta(\varepsilon^{-1} \log (1/\delta))$ non-zero entries in every column while achieving optimal dimension of projected space.
 
Another way to improve the computational time is to use composition of matrices, each of which allows fast computation.  This approach was first taken by Ailon and Chazelle~\cite{AC09}. They used a diagonal matrix in composition with the Walsh-Hadamard  matrix to give $O(n \log n)$ running time mapping. However, the amount of randomness involved to perform the mapping was $O(rn)$. This was improved  by Ailon and Liberty~\cite{AL09, AL13} and Krahmer and Ward~\cite{KW11} in subsequent works. %They used random matrices that satisfies the $\mathsf{RIP}$ of optimal order.    
Ailon and Liberty~\cite{AL09, AL13} achieved a sub-optimal bound of $r=O(\varepsilon^{-4} \log m \log^4 n)$ using projection matrices with $\mathsf{RIP}$ of optimal order. Krahmer and Ward~\cite{KW11} extended their idea to show an optimal bound of $r=O(\varepsilon^{-2} \log m)$. 

\medskip
\noindent {\em Restricted Isometry Property.} In the last decade, there has been increased focus on Restricted Isometry Property due to its relation to compressed sensing~\cite{CT06}. The usual technique to construct a distribution of random matrices that satisfies $\mathsf{RIP}$ is by either choosing the original matrix  from some known class of matrix and sample $r$ row to form $\Phi$, or chosing first row of matrix is chosen at random and form the remaining rows of $\Phi$ deterministically. For example, in
~\cite{CT06, RV08}, the authors chose an orthonormal $n \times n$ Hadamard matrix (or discrete Fourier transform) in the first step and then sample $r$ rows independently at random and proved that this distribution of random matrices satisfies the $\mathsf{RIP}$ if $r \geq \delta^{-2} k \log^4n$. On the other hand, Rauhut {\it et al.}~\cite{RRT10} picked the first row from a Gaussian or Rademacher random vector and construct subsequent row by rotating an element to the right relative to the last row. They showed that sampling $r$ rows subsequently satisfies the $\mathsf{RIP}$ with high probability for $r \geq \max ( \delta^{-1} \sqrt{(k \log n)^3}, \delta^{-2} k \log^4 n )$. 

 %All the traditional {\sf JL} lemma are stated and proven in $\ell_2$ norm. Charikar and Sahai~\cite{CS02} showed an impossibility result for dimension reduction using linear mapping in $\ell_1$ norm, which was extended by Bartal et al~\cite{BRS11}.

%An interesting feature of {\sf JL} transform is its ability to almost characterize the whole Hilbert space. It was shown by Johnson and  Naor~\cite{JN10} that any normed space $\cX$, that satisfies the {\sf JL} lemma, is almost Euclidean in the sense that every $n$-dimensional subspace of $\cX$ embeds in to Hilbert space with distortion at most $2^{O(\log^* n)}$. 


%\subsection{Our Contribution and Comparisons to Previous Works} \label{sec:compare}
 %There are two more works that achieves randomness-efficient fast-JL transform: Ailon and Liberty~\cite{AL13} and Krahmer and Ward~\cite{KW11}.  However, both the work assume that there exists a matrix that satisfies the $\mathsf{RIP}$ bound optimally. Unfortunately, to our knowledge, until now there are no such constructions that uses $O(n)$ random samples and also allows fast transformation, which the paper aims to achieve. Since we have a construction for randomness efficient Johnson-Lindenstrauss lemma which is unconditional, we can invoke Baraniuk {\it et al.}~\cite{BDDW07} to get an matrix that satisfies $\mathsf{RIP}$ bound with optimal sparsity parameters. 
 
%Our bound in the case of random projection allows us to give first construction of random matrix that satisfies restricted isometry property optimally and is fast to compute. Here, we compare our work relative to earlier known constructions that allows fast matrix-vector multiplication and has the $\mathsf{RIP}$. 

%We cover this in more detail in Section~\ref{sec:compressed}. In this sense, we make an unconditional construction. 
\medskip
\noindent {\em Differential Privacy.}  There is a rich literature on differential privacy. Its first formal definition was  given by Dwork {\it et al.}~\cite{DMNS06}. The authors used Laplacian distribution to guarantee differential privacy for bounded {\em sensitivity} query functions. The Gaussian variant of this basic mechanism was proven to preserve differential privacy by 
Dwork {\it et al.}~\cite{DKMMN06} in a follow-up work. Since then, many mechanisms for preserving differential privacy have been proposed in the literature~\cite{BLR08, DRV10, GHRU11, GRU12, KKMM12, HLM12, HR12, MT07, RR10}.  All these mechanisms has one 
common feature: they perturb the output before responding to  queries. Blocki {\it et al.}~\cite{BBDS12, BBDS13} and Upadhyay~\cite{Upadhyay13} took a complementary approach: they perturb the matrix  and perform a random projection on this matrix. 

\subsection{Our Contributions and Techniques}
Like many previous constructions that better the naive construction of {\sf JL} transform, the techniques used in this paper are built around the idea of preconditioning by Ailon and Chazelle~\cite{AC09}. 
Intuitively, this  helps  to get a good concentration bound even when we use limited samples from a Gaussian distribution.
Later, we point out our differences from the construction of Ailon and Chazelle~\cite{AC09}. 

We first summarize the construction of Ailon and Chazelle~\cite{AC09}. The projection matrix used by Ailon and Chazelle~\cite{AC09} is $\Phi=PWD$, where $W$ is the Walsh-Hadamard matrix, $D$ is a diagonal signed Bernoulli matrix, and the matrix $P$ is constructed in the following manner:  every entry $P_{ij}$ is picked from normal distribution $\cN(0,1)$ with probability $p$ and set to $0$ with probability $1-p$.  The parameter $p$ governs the number of non-zero entries in $P$. For the rest of this paper, we call $P$ the projection matrix and $WD$ the smoothening matrix.
Ailon and Chazelle~\cite{AC09} were interested in  reducing the run time of the transformation; therefore, their objective was to keep the expected number of non-zero entries in $P$ bounded. 
On the flip-side, the expected sampling complexity of Ailon and Chazelle~\cite{AC09} is $O(rnp)$, where the mapping is from $n$ to $r$ dimension space.
We diverge from Ailon and Chazelle~\cite{AC09} in the construction of $P$. 
Our aim is to bound the number of distinct entries in the projection matrix; 
therefore, we bound the number of distinct entries.
Our projection matrix also has the same form $PWD$, where $P$ is constructed in a specific manner. 

We first state our first unsuccessful attempt. Recall that our aim is to use minimum number of samplings from various distributions. First attempt could be to pick $n$ Gaussian samples and form the first row of the matrix $P$ and use permutations to form the rest of the rows.  If we use some fixed permutation, we have a variant of partial circulant matrices, which satisfies the $\mathsf{RIP}$ of suboptimal order~\cite{RRT10}. Unfortunately, this is the best bound available and we were unable to improve it any further.

%The second approach could be to fix the set of permutations by some deterministic choice. The utility guarantee is achieved and so is the randomness guarantee; however, we face a subtle issue while proving the differential privacy. The rows of matrix $P$ are not independent; rather they are correlated in a very strong manner, making the analysis extremely cumbersome. 

We use the idea of Krahmer and Ward~\cite{KW11} to randomly permute the rows of the matrix $WD$ using a permutation matrix. However, we still do not achieve the required construction. For this, we use the spherical symmetry of Gaussian matrix, but our crucial observation here is that even a diagonal Gaussian matrix suffices. An intuition why our construction works can be seen from the following observation: any given row of $\Phi'$ formed as above (i.e., composition of diagonal Gaussian matrix, a permutation matrix,  and $WD$ in the order from left to right matrix multiplication) is an i.d.d. Gaussian. This is because, for any row $i$,  entry $\Phi_{ij}'$ consists of a sum of zero-mean independent Gaussian random variables and sign change retains the Gaussian property. Moreover, ${\sf Var}(\Phi')=n$ and $D$ and the random permutation ensures that different entries in the row $i$ have zero correlation. Since, the first and the second moment suffices for Gaussian distribution, we have that every row is i.d.d. Gaussian. Therefore, $\Phi'$ can be seen as ``mimicking" the nature of random dense Gaussian matrices. We then use the idea of Rudelson and Vershynin~\cite{RV08} to sample $r$ rows to form the final projection matrix. Therefore, at the cost of gross oversimplification, an intuitive way to see our construction is as a hybrid of the known constructions of projection matrix with $\mathsf{RIP}$ and known constructions of {\sf JL} transform.


The general idea to prove results of the form stated in~\eqnref{JL} is to first bound the expectation of the random variables corresponding to the output of an application of the transformation matrix, and then use the standard concentration bound to prove the result. For example, in the simplified proof by Dasgupta and Gupta~\cite{DG03}, the above method gives the failure bound of at most $1-1/n$.  The idea is to then repeat the experiment required number of times to get a bound closer to any constant desired. We cannot rely on repetition because it would increase the random samples required. Therefore, we have to give a tighter bound. For this, we rely on a result from statistical model selection. %We use the same idea. 

%We break our analysis in two parts. We first use the result of Ailon and Chazelle~\cite{AC09}, i.e., for any unit vector $\bx$, $WD\bx$ has bounded co-ordinates. In other words, $WD$ smoothens a vector $\bx$ to give a vector $\tilde{\bx}$. Then, we use this promise to prove that when we multiply a diagonal Gaussian matrix from the right after a permutation, then $\tilde{\bx}$ preserves the Euclidean norm with high probability. For this, we use  known concentration inequalities from the area of model selection. Unlike the earlier results on randomness-efficient {\sf JL} transform that uses $\mathsf{RIP}$ of the matrices, the proof in this paper is  elementary and relies on basic concentration inequalities. 

The result for Restricted Isometry follows immediately from~\thmref{BDDW07}. However, the proof of differential privacy is far more involved. It is tempting to assume that multiplying our projection matrix (because of the form it has) results in $r$-multivariate Gaussian and proof of~\cite{BBDS12} can be applied. However, there are subtle correlation between two rows (or two columns) of the projection matrix. Therefore, applying our projection matrix to a private matrix does not yield $n$ independent multivariate distribution, but rather one matrix-variate distribution. We make an adjustment that does not effect our earlier bounds and ease the computation of the resulting distribution. We then prove the resulting distribution of published matrix is differentially private.


==> lra.tex <==
\renewcommand{\X}{\mathbf{X}}
\renewcommand{\K}{\mathbf{K}}
\renewcommand{\S}{\mathbf{S}}
\renewcommand{\bL}{\mathbf{L}}
\renewcommand{\bH}{\mathbf{H}}

\begin{versionA}
The key result that Upadhyay~\cite{Upadhyay14} proved to show the privacy guarantee of their algorithm for computing low-rank approximation is as follows:
\begin{theorem}
	If the singular values of an $m \times n$ input matrix $\bA$ are at least ${\frac{c r \log (2/\beta)}{\alpha}}$, then $\bPhi^{\mathsf T} \bPhi  \bA^{\mathsf T}$, where $\bPhi$ is an $r \times n$ random matrix with entries picked i.i.d. from $\cN(0,1)$, is $(\alpha, \beta)$-differentially private. %It takes $O(mn \log b)$ time and uses linear random samples, where $ b= \min \{ r,c_1 \alpha^{-1} \log(1/\beta) \log(r/\beta) \log((16 \alpha^{-1} \log(1/\beta) \log(r/\beta))/\beta)\}$. 
\end{theorem}
\end{versionA}
For this,~\cite{Upadhyay14} first computed the matrix-variate distribution of the output matrix and then proved privacy. We do not care about normalization factor and terms that would be common for both the neighbouring matrices. In our case, $\bPhi=\bP \bPi \bW \bD$. Moreover,  $\bP^{\mathsf T} \bP$ has the form of block diagonal matrix with each block of the form $\bPhi_i^{\mathsf T} \bPhi_i$ for $\bPhi_i$ as defined in~\figref{basic}. Therefore, we compute the probability density function of each of these blocks. We can then divide the input matrix $\bA$ into $r$ blocks corresponding to $\bPhi_i$.

%We now prove that the second variant preserves privacy if the singular values of the streamed matrix follows the hypothesis of the theorem. 
We first compute the $\PDF$ of the published matrix. %For this, we give two different proofs; the first one is based on the chaining rule, while the second one employs machinery from Borel algebra. 





\renewcommand{\bH}{\mathbf{H}}
\renewcommand{\K}{\mathbf{K}}
\renewcommand{\bL}{\mathbf{L}}

\begin{lemma} \label{lem:pdf}
	Let $\bA$ be a symmetric matrix that is streamed to $\mathsf{PSG}_2$. Let $\bPhi$ be the random Gaussian matrix used in $\mathsf{PSG}_2$, where the rows of $\bPhi$ are formed by $n$-dimensional random Gaussian vectors sampled i.i.d. from $\cN(0,\I)$. Then the probability density function of the output sketch when the whole matrix $\bA$ is streamed is 
	\[ f(\bPhi \bPhi^{\mathsf T}\bA) =c \det( \bSigma \bA)^{-n/2} \exp \paren{ -\tr(\bA^{-1}\bSigma^{-1} \bPhi \bPhi^{\mathsf T}) }. \]
\end{lemma}

This suffices for our purpose because in the proof of differential privacy, we bound the ratio of the probability densities of the output sketch corresponding to the neighbouring matrices. 
\begin{proof}
%\subsubsection{Alternate Proof}
To prove~\lemref{pdf}, we first derive the following general lemma. %Note that we work in the case when the Gaussian matrix is over $\R^{n/r \times 1}$. However, we feel that this general result might be of independent interest.
\begin{lemma} \label{lem:XX}
	Let $\bA$ be a symmetric matrix. Let $\bPhi$ be a rank $r$ Gaussian matrix of dimension $n \times r$ with entries distributed identically. Let $f_\bA(\bPhi)$ be a function of $\bPhi$ which depends only through $\bPhi \bPhi^{\mathsf T}\bA$. Then 
	\[ \int\limits_{\bPhi \bPhi^{\mathsf T}\bA=\K} f_\bA(\bPhi \bPhi^{\mathsf T}\bA) \mathrm{d}\bPhi = c \cdot \det (\K)^{|(n-m-1)|/2} f(\K). \]
\end{lemma}
\begin{proof}
	First note that 
	\begin{align} \int\limits_{\bPhi \bPhi^{\mathsf T}\bA=\K} f_\bA(\bPhi \bPhi^{\mathsf T}) \mathrm{d}\bPhi = f_\bA(\K) \int\limits_{\bPhi \bPhi^{\mathsf T}\bA=\K}  \mathrm{d}\bPhi.  \label{eq:XX} 
	\end{align}
	
	Since $\bA$ is a symmetric matrix, from Cholesky decomposition, we have that $\bA=\mathbf{M} \mathbf{M}^{\mathsf T}$. Now let $ \mathbf{M}^{\mathsf T}\bPhi=\bL \bH$ and $\mathbf{K}=\bL \bL^{\mathsf T}$, where $\bL$ are lower triangular matrices with positive diagonal entries $\ell_{ii} >0$ for all $i$ and $\bH$ are orthogonal matrices. Then the Jacobian of this transformation is 
	\begin{align}  2^{-m}\prod_{i=1}^m  \frac{\ell_{ii}^{(n-i)}  \ell_{ii}'^{(n-i)} g(\bH)}{(\ell_{ii} \ell_{ii}')^{(m-i+1)}} = 2^{-m} \det(\K)^{|n-m+1|/2} g(\bH),  \label{eq:JacobianX} \end{align}
	where $g(\cdot)$ is an invariant measure on a  set of tuples of orthonormal vectors in $\R^n$ known as {\em Steifel manifold}. To complete the proof, we need to compute $\int g(\bH) \mathrm{d}\bH$. The joint variate distribution is % of the entries of $\bPhi$ is 
	\begin{align*}
	 \frac{1}{(2\pi)^{mn/2}} \exp \paren{-\frac{1}{2} \sum_{i=1}^m \sum_{=1}^n  (\mathbf{M}^{\mathsf T}\bPhi)_{ij}^2  } 			&=  \frac{1}{(2\pi)^{mn/2}} \exp \paren{-\frac{1}{2} \tr (\mathbf{M}^{\mathsf T}\bPhi \bPhi^{\mathsf T}\mathbf{M})} \\
	 	& =  \frac{1}{(2\pi)^{mn/2}} \exp \paren{-\frac{1}{2} \tr (\bPhi \bPhi^{\mathsf T}\bA)}.
	\end{align*}
	Now since this is a distribution and recalling that $\mathbf{M}^{\mathsf T}\bPhi=\bL\bH$ with $\bH \bH^{\mathsf T} = \I$, we have the following set of relations.
	\begin{align*}
		1 &= \int \frac{1}{(2\pi)^{mn/2}} \exp \paren{-\frac{1}{2} \tr (\bPhi \bPhi^{\mathsf T}\bA)} \mathrm{d}\bPhi \\
		    &= \frac{1}{(2\pi)^{mn/2}}\idotsint\limits_{\substack{\ell_{ij},  \ell_{ii} \geq 0}} \int\limits_{\bH \bH^{\mathsf T}} \prod_{i=1}^m \ell_{ii}^{n-i} \exp \paren{-\frac{1}{2} \tr (\bL \bL^{\mathsf T})} g(\bH) \mathrm{d}\bH  \prod_{j \leq i} \mathrm{d}\ell_{ij} \\
		    &= \frac{1}{(2\pi)^{mn/2}} \idotsint\limits_{\substack{\ell_{ij},  \ell_{ii} \geq 0}} \int\limits_{\bH \bH^{\mathsf T}} \prod_{i=1}^m \ell_{ii}^{n-i} \exp \paren{-\frac{1}{2} \sum_{j \leq i} \ell_{ij}^2} g(\bH) \mathrm{d}\bH \prod_{j \leq i} \mathrm{d}\ell_{ij} .
	\end{align*} 
	Now since $g(\bH)$ is independent of $\ell_{ij}$'s, we can break the integrals. Now noting the following integral results,
	\[ \int\limits \exp\paren{ - \frac{1}{2} x^2} \mathrm{d}x  = \sqrt{2\pi} \qquad  \text{and} \qquad \int\limits x^{n-i} \exp\paren{ - \frac{1}{2} x^2} \mathrm{d}x  = 2^{|n-m+1|/2} \Gamma \paren{(n-i+1)/2}, \]
	where $\Gamma (\cdot)$ is the gamma function. 
	It follows that  $\int g(\bH) \mathrm{d}\bH = 2^m \pi^{mn/2} / (\Gamma(n/2))$ is a constant, say $c$. 
Using this in~\eqnref{XX} and~\eqnref{JacobianX}, the lemma follows.
\end{proof}
	
%	Recall that in our case $\mathbf{X}$ is simply a $n/r \times 1$ column matrix $\mathbf{g} = \bPhi_i^{\mathsf T}$ with every entries picked i.i.d. from $\cN(0,1)$ for $1 \leq i \leq r$.  
We are now almost done in the proof of~\lemref{pdf} modulo simple computation of the expectation over a measure which is invariant over the Steifel manifold. This is because in the above lemma, we used an invariant measure on Steifel manifold. Therefore, we need a measure which is invariant on such manifolds. One obvious choice is the Borel's measure on $\bPhi \bPhi^{\mathsf T}$. %This is because Borel's measure is very well defined and understood measure. 
Let $h(\cdot)$ be a non-negative Borel measurable function.  Then~\lemref{XX} gives
\begin{align*}
	\E[h(\bPhi \bPhi^{\mathsf T} \bA)] &= \int\limits_{\bPhi \in \R^{n \times r}} h(\bPhi \bPhi^{\mathsf T}\bA) f_\bA(\bPhi \bPhi^{\mathsf T} \bA) \mathrm{d}\bPhi  
	= \int\limits_{\S >0} \int\limits_{\bPhi \bPhi^{\mathsf T}\bA=\S} h(\bPhi \bPhi^{\mathsf T}\bA)  f_\bA(\bPhi\bPhi^{\mathsf T}\bA) \mathrm{d} \bPhi \mathrm{d}\S \\
	&= \int\limits_{\S>0} h(\S) f_\bA(\S) \mathrm{d}\S \int\limits_{\bPhi \bPhi^{\mathsf T}\bA=S} \mathrm{d} \bPhi= c \int\limits_{\S >0} h(\S) \det(\S)^{|m-n+1|/2} f_\bA(\S) \mathrm{d}\S.
\end{align*}
Hence the density of $\S$ is proportional to $\det(\S)^{|m-n+1|/2} f_\bA(\S).$ When $\mathbf{\Phi}$ is spherically distribution with density $f_\bA(\bPhi \bPhi^{\mathsf T})$, then $\bPhi \bPhi^{\mathsf T}$ is distributed as Liouville's distribution of the first kind\footnote{Random variables $\bx_1, \cdots, \bx_r$ are said to have Liouville's distribution of the first kind if their joint probability density function is $\prod \bx_i^{a_i-1} {g}(\sum \bx_i)$, where $\bx_i \in (0,\infty), a_i >0$ and $g$ is a measurable real valued function such that $\int_0^\infty g(\tau) \tau^{s-1} d\tau$ exists for  $s>0$.}. When every entry of $\bPhi$ is sampled from $\cN(0,1)$, then 
\[ f_\bA(\bPhi \bPhi^{\mathsf T}\bA) = c \det( \bSigma \bA)^{-n/2} \exp \paren{ -\tr(\bA^\dagger \bSigma^\dagger  \bPhi \bPhi^{\mathsf T}) }. \]

This completes the proof.
\end{proof}
%It is clear that the Jacobian of $ \bUpsilon \mathbf{A}$ is $\bA$ for any $m \times n/r$ matrix $\mathbf{A}$. Combined with standard transformation method, this immediately gives that the probability density function is proportional to  
%\begin{align}
% \det(\mathbf{A})^{-n/2} \exp \paren{-\frac{1}{2} \tr \paren{ (\mathbf{A})^\dagger   \bUpsilon  }}.  \label{eq:pdf}
% \end{align}




We can now prove~\thmref{PSG2}. Let $\delta_0= \delta/2r$.
Here, we use the notion of neighbouring matrices when $c=1/2$.  Let $\bA$ and $\widetilde{\bA}$ be a pair of neighbouring matrices, i.e., 
%From our definition of neighbouring matrices, $ \bA -\widetilde{\bA}   = \mathbf{E} = {\mathbf{v}}  {\mathbf{e}_i}^{\mathsf T}$ for an unit vector ${\mathbf{v}}$ and some $i$. 
 $\bA -\widetilde{\bA}= (\mathbf{v} \mathbf{e}_i^{\mathsf T} + \mathbf{e}_i \mathbf{v}^{\mathsf T})/2 $, where $\mathbf{v}$ is a unit vector. This would also be the case where we invoke~\thmref{PSG2}. Let $\mathbf{E}=(\mathbf{v} \mathbf{e}_i^{\mathsf T} + \mathbf{e}_i \mathbf{v}^{\mathsf T})/2 $. Let $\bUpsilon = \bPhi \bPhi^{\mathsf T},$ where the rows of $\bPhi$ are formed by $n$-dimensional random Gaussian vectors sampled i.i.d. from $\cN(0,\I).$

Using~\lemref{pdf}, the published matrices corresponding to the two neighbouring matrices $\bA$ and $\widetilde{\bA}$ have the  probability density function proportional to 
\begin{align*}
%	  & \frac{ \exp (-\tr (\bA^\dagger  \bUpsilon )/2) \Delta(\bUpsilon)^{(n-r-1)/2}} {2^{rn/2} \pi^{n(n-1)/4} \Delta(\bA)^{r/2} \prod_{i=1}^r \Gamma((n-i+1)/2)} = C \frac{ \exp (-\tr (\bA^\dagger  \bUpsilon )/2) } { \Delta(\bA)^{r/2} }, \\
%	&   \frac{ \exp (-\tr ((\widetilde{\bA}^\dagger  \bUpsilon )/2) \Delta( \bUpsilon)^{(n-r-1)/2}} {2^{rn/2} \pi^{n(n-1)/4} \Delta(\widetilde{\bA} )^{r/2} \prod_{i=1}^r \Gamma((n-i+1)/2)} = C  \frac{ \exp (-\tr ((\widetilde{\bA}^{\mathsf{T}} \widetilde{\bA})^\dagger  \bUpsilon )/2)} { \Delta(\widetilde{\bA} )^{r/2}}, 
\frac{ \exp (-\tr (\bA^\dagger  \bUpsilon )/2) } { \Delta(\bA)^{r/2} } \qquad \text{and} \qquad  \frac{ \exp (-\tr (\widetilde{\bA}^\dagger  \bUpsilon )/2)} { \Delta(\widetilde{\bA} )^{r/2}}.
\end{align*}
%where $ C= { \Delta( \bUpsilon)^{(n-r-1)/2}}/ \paren{2^{rn/2} \pi^{n(n-1)/4} \prod_{i=1}^r \Gamma((n-i+1)/2)}$.
It is straightforward to see that combination of the following proves $(\varepsilon,\delta)$-differential privacy of the published matrix:
\begin{align} \exp(-\varepsilon/r) \leq \sqrt{\frac{\widetilde{\Delta}(\bA)}{\widetilde{\Delta}(\widetilde{\bA})}} \leq  \exp( \varepsilon/r) \quad \text{and} \quad 
\p \sparen{| \tr \paren{ \paren{ \bA^\dagger  - \widetilde{\bA}^\dagger  } \bUpsilon} |   \leq \varepsilon} \geq 1 -\delta. \label{eq:main}
\end{align} 

Let $\sigma_1\geq \cdots, \geq \sigma_d \geq \sigma_{\mathsf{min}}$ be the singular values of $\bA$. 
 Let $\widetilde{\sigma}_1, \geq \cdots, \geq \widetilde{\sigma}_d \geq \sigma_{\mathsf{min}}$ be the singular value  for $\widetilde{\bA}$. Let $G$ be the set of indices for which $\sigma_i > \widetilde{\sigma}_i$. Since $\bA$ and $\widetilde{\bA}$ are both symmetric and the singular values of $\bA - \widetilde{\bA}$ and $\widetilde{\bA} -\bA$ are the same,  $\sum_{i \in G}(\sigma_i - \widetilde{\sigma}_i) \leq 1$ using~\lemref{lidskii}.  The first bound follows similarly as in Blocki {\it et al.}~\cite{BBDS12}.
 For the second  bound in~\eqnref{main}, we first bound the following
\begin{align*}
 \tr \paren{ \paren{ \bA^\dagger  - \widetilde{\bA}^\dagger  } \bUpsilon}  &=  \tr \paren{ \paren{ \bA^\dagger  (\widetilde{\bA}) (\widetilde{\bA})^\dagger  - \widetilde{\bA}^\dagger  } \bUpsilon} \\
 		&=  \tr \paren{ \paren{ \bA^\dagger  (\bA+\mathbf{E}) \widetilde{\bA}^\dagger  -  \widetilde{\bA}^\dagger  } \bUpsilon}  \\
		&=  \tr \paren{ \paren{ \bA^\dagger  \mathbf{E} \widetilde{\bA}^\dagger  } \bUpsilon }.
 \end{align*}

Using the singular value decomposition of $\bA = \bU \bSigma \bV^{\mathsf{T}}$ and $\widetilde{\bA} = \widetilde{\bU} \widetilde{\bSigma} \widetilde{\bV}^{\mathsf{T}}$, and the fact that $\mathbf{E} = {\mathbf{v}} { \mathbf{e}_i}^{\mathsf T}$ for some $i$, we can further solve the above expression.
\begin{align*}
  \tr \paren{ \paren{ \bA^\dagger  - \widetilde{\bA}^\dagger  } \bUpsilon}  &= \tr \paren{ \paren{ \bA^\dagger  \mathbf{E} \widetilde{\bA}^\dagger  } \bUpsilon }  \\
  	&=\frac{1}{2} \tr \paren{  \bU \bSigma^\dagger  \bV^{\mathsf{T}} {\mathbf{v}} { \mathbf{e}_i}^{\mathsf T} \widetilde{\bU} \widetilde{\bSigma}^\dagger  \widetilde{\bV}^{\mathsf{T}}\bUpsilon }  + \tr \paren{  \bU \bSigma^\dagger  \bV^{\mathsf{T}} {\mathbf{e}_i} { \mathbf{v}}^{\mathsf T} \widetilde{\bU} \widetilde{\bSigma}^\dagger  \widetilde{\bV}^{\mathsf{T}}\bUpsilon }   \\
	&=\frac{1}{2} \sum_{j=1}^r \tr  \paren{ \mathbf{g}^{\mathsf T}_j \bU \bSigma^\dagger  \bV^{\mathsf{T}}  {\mathbf{v}} { \mathbf{e}_i}^{\mathsf T} \widetilde{\bU} \widetilde{\bSigma}^\dagger  \widetilde{\bV}^{\mathsf{T}}\mathbf{g}_j  + \mathbf{g}^{\mathsf T}_j \bU \bSigma^\dagger  \bV^{\mathsf{T}}  {\mathbf{e}_i} { \mathbf{v}}^{\mathsf T} \widetilde{\bU} \widetilde{\bSigma}^\dagger  \widetilde{\bV}^{\mathsf{T}}\mathbf{g}_j }.
  \end{align*}

Fix a $j$. We bound the following.
\begin{equation}
 \left| \tr  \paren{ \mathbf{g}^{\mathsf T}_j \bU \bSigma^\dagger  \bV^{\mathsf{T}}  {\mathbf{v}} { \mathbf{e}_i}^{\mathsf T} \widetilde{\bU} \widetilde{\bSigma}^\dagger  \widetilde{\bV}^{\mathsf{T}}\mathbf{g}_j  + \mathbf{g}^{\mathsf T}_j \bU \bSigma^\dagger  \bV^{\mathsf{T}}  {\mathbf{e}_i} { \mathbf{v}}^{\mathsf T} \widetilde{\bU} \widetilde{\bSigma}^\dagger  \widetilde{\bV}^{\mathsf{T}}\mathbf{g}_j }. \right| .\label{eqn:finalwishart}
\end{equation}

We now look at each term in the above expression. $ \mathbf{g}^{\mathsf T}_j \bU \bSigma^\dagger  \bV^{\mathsf{T}} {\mathbf{e}_i}$ is distributed as $\cN(0, \|  \bU \bSigma^\dagger  \bV^{\mathsf{T}} {\mathbf{e}_i}\|^2)$, 
and ${ \mathbf{v}^{\mathsf T}} \widetilde{\bU} \widetilde{\bSigma}^\dagger  \widetilde{\bV}^{\mathsf{T}}\mathbf{g}_j$ is distributed as $\cN(0, \| { \mathbf{v}^{\mathsf T}} \widetilde{\bU} \widetilde{\bSigma}^\dagger  \widetilde{\bV}^{\mathsf{T}} \|^2)$. Similarly, $ \mathbf{g}^{\mathsf T}_j \bU \bSigma^\dagger  \bV^{\mathsf{T}} {\mathbf{v}}$ is distributed as $\cN(0, \|  \bU \bSigma^\dagger  \bV^{\mathsf{T}} {\mathbf{v}}\|^2)$, 
and ${ \mathbf{e}_i^{\mathsf T}} \widetilde{\bU} \widetilde{\bSigma}^\dagger  \widetilde{\bV}^{\mathsf{T}}\mathbf{g}_j$ is distributed as $\cN(0, \| { \mathbf{e}_i^{\mathsf T}} \widetilde{\bU} \widetilde{\bSigma}^\dagger  \widetilde{\bV}^{\mathsf{T}} \|^2)$.  Since $\mathbf{v}$ and $\mathbf{e}_i$ are unit vectors, the norm of the first the third quantities are less than $ 1/\sigma_{\mathsf{min}},$ and that of second and fourth is less than $1+1/ \sigma_{\mathsf{min}}$, respectively. 
Therefore, from the concentration inequality of Gaussian distribution, we have 
\begin{align*} \p \sparen{ (\ref{eqn:finalwishart}) \leq 2 \paren{\frac{1}{ \sigma_{\mathsf{min}}} + \frac{1}{ \sigma_{\mathsf{min}}^2}} \ln (4/\delta_0) \leq \varepsilon } \geq 1- \delta_0. \end{align*}

Taking union bound, we have  with probability $1-\delta$, $-\varepsilon \leq \tr \paren{ \paren{ \bA^\dagger  - \widetilde{\bA}^\dagger  } \bUpsilon} \leq \varepsilon$.







The rest of the proof now follows similarly as in the gaussian case of~\cite{Upadhyay14} after adjusting the way we adjusted in the proof of~\thmref{DP}. More specifically, let  $\bA = \bU \bSigma \bV^{\mathsf{T}}$  be the singular value decomposition of $\bA$. Recall that $\bP^{\mathsf T} \bP$ has the following form:
\[
\begin{pmatrix}
	\bPhi_1^{\mathsf T} \bPhi_1 & \mathbf{0} & \cdots & \mathbf{0} \\
	\mathbf{0} & \bPhi_2^{\mathsf T} \bPhi_2 & \cdots & \mathbf{0} \\
	\vdots & \ddots & \ddots & \vdots \\
	\mathbf{0} & \mathbf{0} & \cdots &\bPhi_r^{\mathsf T} \bPhi_r
\end{pmatrix}.
\]

Note that we are computing $\bPhi^{\mathsf T} \bPhi \bA^{\mathsf T}= \bD^{\mathsf T} \bW^{\mathsf T} \bPi^{\mathsf T} \bP^{\mathsf T} \bP \bPi \bW \bD \bA^{\mathsf T}. $ We can assume that $\bD^{\mathsf T} \bW^{\mathsf T} \bPi^{\mathsf T}$ are post-processing. This is because $\bPi$ just permutes $\bP^{\mathsf T} \bP \bPi \bW \bD \bA^{\mathsf T}$  and $\bD$ either just change the sign of the rows or not depending if $\bD_{ii}$ is $-1$ or $1$. In what follows, we concentrate on proving that $ \bP^{\mathsf T} \bP \bPi \bW \bD \bA^{\mathsf T} = \bP^{\mathsf T} \bP \bPi \bW \bD \bV^{\mathsf T} \bSigma \bU$ preserves differential privacy. From~\lemref{zero}, we know that if we divide $\bV$ into blocks of $n/r$ rows, then none of the rows are all zero row with probability at least $1-2^{-\Omega((1-\theta)^2n^{2/3})}$. Therefore, as before, we break $\bPi \bW \bD \bV^{\mathsf T}$ into $r$ blocks of $n/r$ rows each, $\bV_1^{\mathsf T} = ( \bPi \bW \bD \bV^{\mathsf T})_1, \cdots , \bV^{\mathsf T}_r= ( \bPi \bW \bD \bV^{\mathsf T})_r$. Then we can write the output of $ \bP^{\mathsf T} \bP \bPi \bW \bD \bA^{\mathsf T}$ as following:
\[ 
\begin{pmatrix} 
	 \bPhi^{\mathsf T}_1 \bPhi_1  (\bPi \bW \bD \bV^{\mathsf T})_1 \bSigma \bU \\ 
	 \vdots \\ 
	 \bPhi^{\mathsf T}_r \bPhi_r (\bPi \bW \bD \bV^{\mathsf T})_r \bSigma \bU 
\end{pmatrix} =
\begin{pmatrix} 
  \bPhi^{\mathsf T}_1 \bPhi_1 \bV_1 \bSigma \bU \\ \vdots \\ \bPhi^{\mathsf T}_1 \bPhi_1  \bV_r \bSigma \bU
\end{pmatrix}. \]

We can now prove the privacy guarantee. Let $\alpha_0=\alpha/r,\beta_0= \beta/r$.
Let $\bA$ and $\widetilde{\bA}$ be a pair of neighbouring matrices that form the stream. From our definition of neighbouring matrices, $ \bA -\widetilde{\bA}   = \bE = \mathbf{v}  \mathbf{e}_j^{\mathsf T}$ for an unit vector $\mathbf{v}$ and some $j$. We now prove that the output distribution of $\bPhi_i^{\mathsf T} \bPhi_i \bV_i \bSigma \bU$ for any $1 \leq i \leq r$ satisfies $(\alpha_0,\beta_0)$ differential privacy. For any $1 \leq i \leq r$,~\eqnref{pdf} gives that the $i$-th row of the published matrices corresponding to the two neighbouring matrices have the following probability density function
\begin{align*}
	\PDF( \bPhi_i^{\mathsf T}\bPhi_i; \bV_i^{\mathsf{T}} \bSigma^2 \bV_i) &=   
	%\frac{ \exp (-\tr ((\bA^{\mathsf{T}} \bA)^{-1} \bPhi )/2) \beta(\bPhi)^{(n-r-1)/2}} {2^{rn/2} \pi^{n(n-1)/4} \beta(\bA^{\mathsf{T}}\bA)^{r/2} \prod_{i=1}^r \Gamma((n-i+1)/2)} = 
	C \frac{ \exp (-\tr ((\bV_i^{\mathsf{T}} \bSigma^2 \bV_i)^{-1} \bPhi_i^{\mathsf T} \bPhi_i )/2) } { \det(\bV_i^{\mathsf{T}} \bSigma^2 \bV_i)^{1/2} }, \\
	\PDF( \bPhi_i^{\mathsf T} \bPhi_i; \widetilde{\bV}_i^{\mathsf{T}} \widetilde{\bSigma}^2 \widetilde{\bV}_i ) &= 
	%  \frac{ \exp (-\tr ((\widetilde{\bA}^{\mathsf{T}} \widetilde{\bA})^{-1} \bPhi )/2) \beta( \bPhi)^{(n-r-1)/2}} {2^{rn/2} \pi^{n(n-1)/4} \beta(\widetilde{\bA}^{\mathsf{T}} \widetilde{\bA} )^{r/2} \prod_{i=1}^r \Gamma((n-i+1)/2)} = 
	C  \frac{ \exp (-\tr ((\widetilde{\bV}_i^{\mathsf{T}} \widetilde{\bSigma}^2 \widetilde{\bV}_i )^{-1} \bPhi_i^{\mathsf T} \bPhi_i )/2)} { \det(\widetilde{\bV}_i^{\mathsf{T}} \widetilde{\bSigma}^2 \widetilde{\bV}_i )^{1/2}}, 
\end{align*}
where $ C= { \det(\bPhi_i^{\mathsf T} \bPhi_i)^{n/2r}}$.

Let us fix an $1 \leq i \leq r$. Let $\sigma_1\geq \cdots, \geq \sigma_m \geq \sigma_{\mathsf{min}}$ be the singular values of $A$. 
 Let $\widetilde{\sigma}_1, \geq \cdots, \geq \widetilde{\sigma}_m \geq \sigma_{\mathsf{min}}$ be the singular value  for $\widetilde{\bA}$. Since the singular values of $\bA - \widetilde{\bA}$ and $\widetilde{\bA} -\bA$ are the same,  $\sum_{i \in G}(\sigma_i - \widetilde{\sigma}_i) \leq 1$ using the Linskii's theorem, where $G$ is the set of indices for which $\sigma_i > \widetilde{\sigma}_i$. The first bound follows similarly as in~\thmref{DP}. 
\begin{align}
\sqrt{\frac{\det(\widetilde{\bV}_i \widetilde{\bSigma}^2 \widetilde{\bV}_i^{\mathsf T}) } {\det(\bV_i \bSigma^2 \bV_i^{\mathsf T})}}  = \sqrt{\prod_i \frac{\widetilde{\sigma}_i^2}{\sigma_i^2}} \leq \exp \paren{\frac{\alpha}{16 r \log (2/\beta)\ln(4/\beta)} }\sum_i (\widetilde{\sigma}_i - \sigma_i) \leq \exp \paren{\alpha_0/2}. \label{eq:main1} 
\end{align}

In the second step, we prove the following:
\begin{align} 
\p \sparen{ \left| \tr \paren{ \paren{ ((\bV_i^{\mathsf{T}} \bSigma^2 \bV_i)^{-1} - (\widetilde{\bV}_i^{\mathsf{T}} \widetilde{\bSigma}^2 \widetilde{\bV}_i)^{-1} }  \bPhi_i^{\mathsf T}\bPhi_i} \right|   \leq \alpha_0} \geq 1 -\beta_0. \label{eq:main2}
\end{align} 

For the second  bound required for the privacy, we first bound the following
\begin{align*}
& \tr \paren{ \paren{ (\bV_i \bSigma^2 \bV_i^{\mathsf T})^{-1} - (\widetilde{\bV}_i^{\mathsf{T}} \widetilde{\bSigma}^2 \widetilde{\bV}_i)^{-1} } \bPhi_i^{\mathsf T} \bPhi_i} \\
& \qquad =  \tr \paren{ \paren{ (\bV_i \bSigma^2 \bV_i^{\mathsf T})^{-1} (\widetilde{\bV}_i \widetilde{\bSigma}^2 \widetilde{\bV}_i^{\mathsf T}) (\widetilde{\bV}_i \widetilde{\bSigma}^2 \widetilde{\bV}_i^{\mathsf T})^{-1} - (\widetilde{\bV}_i \widetilde{\bSigma}^2 \widetilde{\bV}_i^{\mathsf T})^{-1} }  \bPhi_i^{\mathsf T} \bPhi_i} \\
 		& \qquad =  \tr \paren{ \paren{ (\bV_i \bSigma^2 \bV_i^{\mathsf T})^{-1} (\bU \bSigma \bV_i^{\mathsf T} +\bE)^{\mathsf{T}} (\bU \bSigma \bV_i^{\mathsf T} +\bE) (\widetilde{\bV}_i \widetilde{\bSigma}^2 \widetilde{\bV}_i^{\mathsf T})^{-1} - (\widetilde{\bV}_i \widetilde{\bSigma}^2 \widetilde{\bV}_i^{\mathsf T})^{-1} }  \bPhi_i^{\mathsf T} \bPhi_i} \\
		& \qquad =  \tr \paren{ \paren{ (\bV_i \bSigma^2 \bV_i^{\mathsf T})^{-1} (\bV_i \bSigma \bU^{\mathsf T} \bE + \bE^{\mathsf{T}}\widetilde{\bU} \widetilde{\bSigma} \widetilde{\bV}_i^{\mathsf T}) (\widetilde{\bV}_i \widetilde{\bSigma}^2 \widetilde{\bV}_i^{\mathsf T})^{-1} }  \bPhi_i^{\mathsf T} \bPhi_i }.
 \intertext{Recall that $\bE = \mathbf{v} \mathbf{e}_j^{\mathsf T}$ for some $j$. We divide $\bE$ (i.e., the unit vector $\mathbf{v}$) in the form of $r$ blocks of $n/r$ entries to write $(\bE_1 = \mathbf{v}_1 \mathbf{e}_j^{\mathsf T} , \cdots \bE_r = \mathbf{v}_r \mathbf{e}_j^{\mathsf T})$. we can further solve the above expression.}
 & \tr \paren{ \paren{ (\bV_i \bSigma^2 \bV_i^{\mathsf T})^{-1} - (\widetilde{\bV}_i^{\mathsf{T}} \widetilde{\bSigma}^2 \widetilde{\bV}_i)^{-1} } \bPhi_i^{\mathsf T} \bPhi_i} \\
 & \qquad = \tr \paren{ \paren{ \bV_i \bSigma^{-1} \bU^{\mathsf{T}} \mathbf{e}_j \mathbf{v}_i^{\mathsf T} \widetilde{\bV}_i \widetilde{\bSigma}^{-2} \widetilde{\bV}_i^{\mathsf{T}} + \bV_i \bSigma^{-2} \bV_i^{\mathsf{T}} \mathbf{v}_i \mathbf{e}_j\widetilde{\bU} \widetilde{\bSigma}^{-1} \widetilde{\bV}_i^{\mathsf{T}} } \bPhi_i^{\mathsf T} \bPhi_i}  \\
  &\qquad = \tr \paren{  \bV_i \bSigma^{-1} \bU^{\mathsf{T}} \mathbf{e}_j \mathbf{v}_i^{\mathsf T} \widetilde{\bV}_i \widetilde{\bSigma}^{-2} \widetilde{\bV}_i^{\mathsf{T}} \bPhi } + \tr \paren{\bV_i \bSigma^{-2} \bV_i^{\mathsf{T}} \mathbf{v}_i \mathbf{e}_j\widetilde{\bU} \widetilde{\bSigma}^{-1} \widetilde{\bV}_i^{\mathsf{T}}  \bPhi_i^{\mathsf T} \bPhi_i }  .
%	&= \sum_{j=1}^r \tr  \paren{ \bra{\mathbf{g}_j} \bV \bSigma^{-1} U^{\mathsf{T}} \mathbf{e}_j \mathbf{v}_i^{\mathsf T} \widetilde{\bV}_i \widetilde{\bSigma}^{-2} \widetilde{\bV}_i^{\mathsf{T}} \ket{\mathbf{g}_j} }\\ 
%	& \qquad +  \sum_{j=1}^r \tr \paren{\bra{\mathbf{g}_j}\bV \bSigma^{-2} \bV^{\mathsf{T}} \mathbf{v}_i \mathbf{e}_j\widetilde{\bU} \widetilde{\bSigma}^{-1} \widetilde{\bV}_i^{\mathsf{T}}\ket{\mathbf{g}_j} }.
  \end{align*}
Now using the fact that trace is invariant under cyclic permutation, we have
\begin{equation}
 \left| \tr  \paren{  \bPhi_i \bV \bSigma^{-1} \bU^{\mathsf{T}} \mathbf{e}_j \mathbf{v}_i^{\mathsf T} \widetilde{\bV}_i \widetilde{\bSigma}^{-2} \widetilde{\bV}_i^{\mathsf{T}}  \bPhi_i^{\mathsf T} } 
	 +  \tr \paren{ \bPhi_i \bV \bSigma^{-2} \bV^{\mathsf{T}} \mathbf{v}_i \mathbf{e}_j\widetilde{\bU} \widetilde{\bSigma}^{-1} \widetilde{\bV}_i^{\mathsf{T}}  \bPhi_i^{\mathsf T} } \right| .\label{eqn:final}
\end{equation}

We now look at each term in the above expression. $\bPhi_i\bV \bSigma^{-2} \bV^{\mathsf{T}} \mathbf{v}_i$ is distributed as $\cN(0, \| \bV \bSigma^{-2} \bV^{\mathsf{T}} \mathbf{v}_i \|^2)$, $\mathbf{v}_i^{\mathsf T} \widetilde{\bV}_i \widetilde{\bSigma}^{-2} \widetilde{\bV}_i^{\mathsf{T}} \bPhi_i^{\mathsf T}$ as $\cN(0, \|\mathbf{v}_i^{\mathsf T} \widetilde{\bV}_i \widetilde{\bSigma}^{-2} \widetilde{\bV}_i^{\mathsf{T}} \|^2)$, $ \bPhi_i V \bSigma^{-1} \bU^{\mathsf{T}} \mathbf{e}_j$ as $\cN(0, \|  \bV \bSigma^{-1} \bU^{\mathsf{T}} \mathbf{e}_j\|^2)$, 
and $\mathbf{e}_j\widetilde{\bU} \widetilde{\bSigma}^{-1} \widetilde{\bV}_i^{\mathsf{T}}\bPhi_i^{\mathsf T}$ as $\cN(0, \| \mathbf{e}_j\widetilde{\bU} \widetilde{\bSigma}^{-1} \widetilde{\bV}_i^{\mathsf{T}} \|^2)$. Since $\|\mathbf{v}_i \|_2 \leq \|\mathbf{v} \|_2 = 1$ and $\mathbf{e}_i$ is a unit vector, the norm of the above four quantities are less than $1/ \sigma_{\mathsf{min}}^2, 1/ \sigma_{\mathsf{min}}^2+1/ \sigma_{\mathsf{min}}^3, 1/\sigma_{\mathsf{min}},$ and $1/ \sigma_{\mathsf{min}}+1/ \sigma_{\mathsf{min}}^2$, respectively. 

Therefore, from the concentration inequality of Gaussian distribution, we have 
\begin{align*} \p \sparen{ (\ref{eqn:final}) \leq 2 \paren{\frac{1}{ \sigma_{\mathsf{min}}^2} + \frac{1}{ \sigma_{\mathsf{min}}^3}} \ln (4/\beta_0) \leq \alpha } \geq 1- \beta_0. \end{align*}
This is exactly what we wanted to prove.
Combining~\eqnref{main1} and~\eqnref{main2} with~\lemref{zero} gives us~\thmref{DP2}. %Note that here we cannot use~\thmref{DRV10} because there are subtle dependencies between any two rows of the matrix $\bPhi^{\mathsf T} \bPhi$.

